Selective Forgetting: Advancing Machine Unlearning Techniques and Evaluation in Language Models

This paper explores Machine Unlearning (MU), an emerging field that is gaining increased attention due to concerns about neural models unintentionally remembering personal or sensitive information. We present SeUL, a novel method that enables selective and fine-grained unlearning for language models. Unlike previous work that employs a fully reversed training objective in unlearning, SeUL minimizes the negative impact on the capability of language models, particularly in terms of generation. Furthermore, we introduce two innovative evaluation metrics, sensitive extraction likelihood (S-EL) and sensitive memorization accuracy (S-MA), specifically designed to assess the effectiveness of forgetting sensitive information. In support of the unlearning framework, we propose efficient automatic online and offline sensitive span annotation methods. The online selection method, based on language probability scores, ensures computational efficiency, while the offline annotation involves a two-stage LLM-based process for robust verification. In summary, this paper contributes a novel selective unlearning method (SeUL), introduces specialized evaluation metrics (S-EL and S-MA) for assessing sensitive information forgetting, and proposes automatic online and offline sensitive span annotation methods to support the overall unlearning framework and evaluation process.

==> figures/oracle_epoch.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/epoch_125m_oracle.pdf}
% \vskip -0.5em
\caption{\label{fig:oracle_epoch} Trends of S-MA and S-EL scores across epochs for unlearning methods with (i.e., \shortname$^{Oracle}$) and without (i.e., \shortname) oracle annotation.}
% \vskip -0.5em
\end{figure}

==> sections/commands.tex <==
\newcommand\BibTeX{B\textsc{ib}\TeX}

\newcommand{\ours}{\textsc{SciFact}\xspace}
\newcommand{\oursClosed}{$\ours_{\mathrm{closed}}$\xspace}
\newcommand{\oursOpen}{$\ours_{\mathrm{open}}$\xspace}

% System name
\newcommand{\sysname}{\textsc{VeriSci}\xspace}


\newcommand{\fever}{\textsc{Fever}\xspace}
\newcommand{\eraser}{\textsc{ERASER}\xspace}
\newcommand{\snopes}{UKP Snopes\xspace}

% \newcommand\dw[1]{{\color{blue}\{\textit{#1}\}$_{DW}$}}
\newcommand\dw[1]{{\color{blue} #1}}
\newcommand\old[1]{{\color{red} #1}}
\newcommand\ac[1]{{\color{teal}\{\textit{#1}\}$_{AC}$}}
\newcommand\kyle[1]{{\color{orange}\{\textit{#1}\}$_{kyle}$}}
\newcommand\klcomment[1]{{\color{orange}\{\textit{#1}\}$_{kyle}$}}
\newcommand\lucy[1]{{\color{purple}\{\textit{#1}\}$_{lucy}$}}
\newcommand{\hanna}[1]{\textcolor{cyan}{[#1]}}
\newcommand\peter[1]{{\color{purple}\{\textit{#1}\}$_{peter}$}}


\newcommand\todoit[1]{{\color{red}\{TODO: \textit{#1}\}}\xspace}
\newcommand\todo{{\color{red}{TODO}}\xspace}
\newcommand\needcite{{\color{red}{CITE}}\xspace}

\newcommand{\supported}{\textsc{Supported}\xspace}
\newcommand{\refuted}{\textsc{Refuted}\xspace}

% Easier to do supports / refutes instead of supported / refuted
\newcommand{\supports}{\textsc{Supports}\xspace}
\newcommand{\refutes}{\textsc{Refutes}\xspace}
% \newcommand{\notenough}{\textsc{NotEnoughInfo}\xspace}
\newcommand{\notenough}{\textsc{NoInfo}\xspace}

\newcommand{\psupports}{\textsc{PartiallySupports}\xspace}
\newcommand{\prefutes}{\textsc{PartiallyRefutes}\xspace}
\newcommand{\ppartial}{\textsc{Partial}\xspace}

\newcommand{\support}{\textsc{Support}\xspace}
\newcommand{\refute}{\textsc{Refute}\xspace}



% Stance / entailment
\newcommand{\entailment}{entailment\xspace}
\newcommand{\Entailment}{Entailment\xspace}

% URL placeholder
\newcommand{\webpage}{\url{www.placeholder.com}}

% Dataset counts
\newcommand{\numclaims}{1,409\xspace}
\newcommand{\numpapers}{5,183\xspace}
\newcommand{\numevidence}{486\xspace}
\newcommand{\numcitednoevidence}{255\xspace}

% Coarse-grained agreement stats.
\newcommand{\labelkappa}{0.75\xspace} % Cohen's kappa for label agreement.
\newcommand{\labelhumanacc}{0.83\xspace} % Human-human label accuracy.
\newcommand{\rationalekappaagree}{0.71\xspace} % Rationale Cohen's kappa given label agreement.
\newcommand{\rationalekappaoverall}{0.63\xspace} % Rationale Cohen's kappa overall.
\newcommand{\rationalekappabackground}{0.45\xspace} % Rationale for background sentences.
\newcommand{\foneagree}{0.75\xspace}              % Human-huamn F1 given label agreement.
\newcommand{\foneoverall}{0.67\xspace}           % Human-human F1 overall.
\newcommand{\nagreement}{232\xspace}              % Number of claims annotated for coarse-grained agreement.

% Fine-grained agreement stats.
\newcommand{\labelkappafine}{0.48\xspace} % Cohen's kappa for fine-grained label.
\newcommand{\nagreementfine}{224\xspace}              % Number of claims annotated for coarse-grained agreement.


% Modeling performance
\newcommand{\bestpipeline}{0.47\xspace}


% Support levels.
\newcommand{\sfull}{\textsc{FullSupport}\xspace}
\newcommand{\spart}{\textsc{PartialSupport}\xspace}
\newcommand{\rfull}{\textsc{FullRefute}\xspace}
\newcommand{\rpart}{\textsc{PartialRefute}\xspace}

\newcommand{\scoarse}{\textsc{Support}\xspace}
\newcommand{\rcoarse}{\textsc{Refute}\xspace}

\newcommand{\primary}{\textsc{Primary}\xspace}
\newcommand{\supplemental}{\textsc{Supplemental}\xspace}

% Models
\newcommand{\bert}{\textsc{BERT}\xspace}
\newcommand{\scibert}{\textsc{SciBERT}\xspace}
\newcommand{\roberta}{RoBERTa\xspace}
\newcommand{\bioroberta}{BioMedRoBERTa\xspace }
\newcommand{\robertabase}{RoBERTa-base\xspace}
\newcommand{\robertalarge}{RoBERTa-large\xspace}

\newcommand{\softmax}{\textsc{SoftMax}}
\newcommand{\sigmoid}{\textsc{Sigmoid}}

% BERT components
\newcommand{\cls}{\textsc{CLS}\xspace}
\newcommand{\sep}{\textsc{SEP}\xspace}


\newcommand{\multistage}{\textsc{Multistage}\xspace}


\newcommand{\multinli}{\textsc{MultiNLI}\xspace}
\newcommand{\zeroshot}{\textsc{ZeroShot}\xspace}

\newcommand{\nse}{\textsc{NoScoreEv}\xspace}
\newcommand{\se}{\textsc{ScoreEv}\xspace}


% Subsets of the corpus
\newcommand{\Dcited}{\cD_{\mathrm{cited}}}
\newcommand{\Dseed}{\cD_{\mathrm{seed}}}
\newcommand{\Ddecoy}{\cD_{\mathrm{decoy}}}
\newcommand{\dcited}{\bd_{\mathrm{cited}}}
\newcommand{\dseed}{\bd_{\mathrm{seed}}}
\newcommand{\dciting}{\bd_{\mathrm{citing}}}
\newcommand{\sciting}{\bs_{\mathrm{citing}}}


% negation anecdotes
\newcommand{\fracSupportIncrease}{9\% \xspace}
\newcommand{\fracSupportReduce}{5\% \xspace}
\newcommand{\fracRefuteIncrease}{12\% \xspace}
\newcommand{\fracRefuteReduce}{6\% \xspace}

% FEVER classification
\newcommand{\bestFeverRetrieval}{0.80 \xspace}
\newcommand{\bestFeverEntailment}{0.90 \xspace}

\newcommand{\feverPaperEntailment}{0.88 \xspace}

% Math
\newcommand{\yhat}{\widehat{y}}
\newcommand{\rhat}{\widehat{r}}
\newcommand{\Rhat}{\widehat{R}}
\newcommand{\Shat}{\widehat{S}}
\newcommand{\shat}{\widehat{s}}
\newcommand{\rstar}{r^*}
\newcommand{\Sstar}{S^*}
\newcommand{\Ehat}{\widehat{\cE}}
\newcommand{\Estar}{\cE^*}
\newcommand{\ahat}{\widehat{a}}

% Colors and check marks
\definecolor{NiceGreen}{RGB}{125,204,110}
\definecolor{NiceRed}{RGB}{222,0,0}
\definecolor{c1}{rgb}{0.12, 0.46, 0.70}
\definecolor{c2}{rgb}{1.0, 0.50, 0.05}
\definecolor{c3}{rgb}{0.17,0.63,0.17}

\newcommand{\cmark}{{\color{NiceGreen} \ding{51}}} % Green check mark.
\newcommand{\xmark}{{\color{NiceRed} \ding{55}}}  % Red x.

\newcommand{\best}{\textsc{Best}\xspace}

% F1
\newcommand{\fonecoarse}{$F1_{\textrm{abstract}}$\xspace}
\newcommand{\foneAbstLab}{$F1_{\textsc{A,L}}$\xspace}
\newcommand{\foneAbstRat}{$F1_{\textrm{A,R}}$\xspace}
\newcommand{\fonefine}{$F1_{\textrm{sentence}}$\xspace}
\newcommand{\foneRatSel}{$F1_{\textrm{R,S}}$\xspace}
\newcommand{\foneRatLab}{$F1_{\textrm{R,L}}$\xspace}

\newcommand{\abstractLabelOnly}{$\textrm{Abstract}_{\textrm{Label-Only}}$\xspace}
\newcommand{\abstractLabelRationale}{$\textrm{Abstract}_{\textrm{Label+Rationale}}$\xspace}
\newcommand{\sentenceSelectionOnly}{$\textrm{Sentence}_{\textrm{Selection-Only}}$\xspace}
\newcommand{\sentenceSelectionLabel}{$\textrm{Sentence}_{\textrm{Selection+Label}}$\xspace}



% Website
\newcommand{\website}{\url{https://github.com/allenai/scifact}}

% Model component abbreviations
\newcommand{\abst}{\textrm{abst}\xspace}
\newcommand{\rtnl}{\textrm{rtnl}\xspace}
\newcommand{\lbl}{\textrm{lbl}\xspace}


% Pipeline components
\newcommand{\componentone}{\textsc{AbstractRetrieval}\xspace}
\newcommand{\componenttwo}{\textsc{RationaleSelection}\xspace}
\newcommand{\componentthree}{\textsc{LabelPrediction}\xspace}

% Table commands
\newcommand{\thinmid}{\arrayrulecolor{black!30}\midrule}
\newcommand{\thickmid}{\arrayrulecolor{black}\midrule}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% Supports and refutes
% \definecolor{c1}{RGB}{84,130,53}
\definecolor{c1}{RGB}{21,156,0}
% \newcommand{\supportsCovid}[1]{{\color{c1} \textbf{#1}}}
\newcommand{\supportsCovid}[1]{{\color{c1} {#1}}}

\definecolor{c2}{RGB}{218,0,0}
% \newcommand{\refutesCovid}[1]{{\color{c2} \textbf{#1}}}
\newcommand{\refutesCovid}[1]{{\color{c2} {#1}}}

\definecolor{c3}{RGB}{127,127,127}
\newcommand{\wrongContext}[1]{{\color{c3} \textbf{#1}}}


% Highlight color
\definecolor{lightblue}{RGB}{212, 235, 255}
\definecolor{lightpink}{RGB}{255,192,203}
\definecolor{lightgreen}{RGB}{177, 231, 171}
\definecolor{lightyellow}{RGB}{255, 255, 148}
\sethlcolor{lightblue}

\newcommand\hlc[2]{\sethlcolor{#1} \hl{#2}}

==> sections/dataset_construction.tex <==
\section{Dataset Construction}


\subsection{Previous Unlearning Evaluation}
\cite{patil2023can} evaluate the unlearning performance on two factual completion dataset CounterFact \cite{meng2022locating} and zsRE \cite{levy2017zero} to evaluate the unlearning performance by comparing the accuracy score before and after the data point deleting (i.e., $\Delta$-Acc). For example, the factual completion task aims to answer ``The Autonomous University Of Madrid Is In'' with ``Spain''. Though it could be regarded a simple question-answering problem, these two datasets are not the target of this work, as we focus more on the privacy leakage in longer generated sentences. 

\cite{jang2022knowledge} conduct experiments on 9 classification (commonsense reasoning, e.g., Hellaswag \cite{zellers2019hellaswag}) datasets and 4 dialogue datasets (scientific reasoning, e.g., MathQA \cite{amini2019mathqa}), and propose a new unlearning evaluation metrics named Extraction Likelihood (EL) and adopt a metric called Memorization Accuracy (MA) from \cite{tirumala2022memorization}. EL measures the average success rate of varying extraction attacks quantified via getting the n-gram overlap of generated and target token sequences. MA measures how model has memorized the given token sequences. These two evaluation metrics reflect the model's performance handling extraction attack and further indicate effectiveness of the unlearning algorithms (e.g., smaller EL and MA scores after unlearning indicate that the unlearning is more effective as the unlearned model can better handle the extraction attack).

\cite{wang-etal-2023-kga} conducts experiments on three representative datasets LEDGAR \cite{tuggener2020ledgar}, IWSLT14 German-English \cite{cettolo2014report} and PersonaChat \cite{zhang2018personalizing} to evaluate the unlearning performance for classification, translation and generation tasks, separately. \cite{wang-etal-2023-kga} adopts Jensen–Shannon Divergence (JSD), Language model Probability Distance (LPD), and Proportion of instances with Decreased Language model Probability (PDLP) to evluate the unlearning effectiveness, where LPD and PDLP are calculated based on comparing the results of unlearning to original model. The scores of LPD and PDLP are not either the larger the better nor the smaller the better. \cite{wang-etal-2023-kga} regards the scores of LPD and PDLP which are closer to the performance of ReTrain model (i.e., retraining the model from scratch after removing the data to be forgotten from original training set). Such evaluation methods highly relies on the availability of ReTrain model, while the retrain models are unavailable to get or costly to get (e.g., LLM's retraining for unlearning evaluation is impractical).

We summarize the aforementioned unlearning evaluation with the following characteristics:

\paragraph{Indirect evaluation.} Due to the un-well defined and standard unlearning targets, most of the previous research adopt indirect evaluation metrics to compare the evaluation scores changes (e.g., accuracy changes in \cite{patil2023can}, extraction likelihood in \cite{jang2022knowledge} and language probability in \cite{wang-etal-2023-kga}) before and after the unlearning. Besides, 

\paragraph{Privacy unrelated.} Though machine unlearning is strongly motivated from the privacy issue that existed in data-intensive neural networks, most of the previous work evaluate the unlearning based on non-user related datasets. These datasets themselves does not contain user-related information. For instance, \cite{jang2022knowledge} explore commonsense and scientific reasoning datasets. An exception is that \cite{wang-etal-2023-kga} employ PersonaChat dataset \cite{zhang2018personalizing} where personalization information is provided for dialogues.

Apart from the aforementioned unlearning evaluation without constrained forgetting data (i.e., the data to be forgotten is randomly sampled), there are also works that limit the data to be forgotten as data with specific attributes (e.g., toxic data \cite{}, biased data \cite{yu2023unlearning}). The evaluation of such unlearning is more straightforward by comparing the corresponding attribute scores (e.g., ) of models before and after unlearning. Unlearning work in this category also meets the two characteristics (i.e., indirect evaluation and privacy unrelated) we summarized. 

\subsection{Dataset Construction Considerations}
In this work, we aim to propose unlearning privacy metrics together with evaluation datasets as complementary to the previous developed evaluation methods. We want to develop datasets that are directly related to user privacy issue instead of public and commonsense. Considering that privacy information 

In \cite{brown2022does} 

\paragraph{Generation Sensitive Information Annotation}

\paragraph{Audience-Specific Sensitive Information Annotation}

\paragraph{Suffix Sensitive Information Information}




\subsection{Automatic and Human Annotation}
We conduct both automatic and human efforts to annotate the sensitive span. 

\subsubsection{Base Datasets Selection} The selection of base datasets are associated with the following two considerations. (1) To have a comparison with the previous work, we select some datasets from the previous work and further annotate sensitive spans based on these datasets. (2) As the user directly related datasets are largely ignored in the previous work, we introduce some user-related datasets with specific user id to assistant the exploration of privacy range. Therefore, we do annotation on the following 8 datasets, each with 2000 instances (i.e., single instances for classification task, source-target sequence pairs for generation task, conversation threads for dialogues) in automatic annotation and . 

Due to there are less explorations on the audience-specific privacy 


\textit{Pile-S1000}: To better assess the unlearning on large language model, we also select instances from dataset Pile \cite{gao2020pile} that is widely adopted in large language model training. We follow the previous work \cite{jang2022knowledge}, we randomly sample 1000 instances for sensitive information annotation from the Training Data Extraction Challenge\footnote{\url{https://github.com/google-research/lm-extraction-benchmark}} (each are 200 token sequences long) from 16 different domains of the Pile corpora \cite{gao2020pile} that are identified to be somewhat easy-to-extract are provided.

\textit{PersonaChat-S1000}: The original PersonaChat \cite{zhang2018personalizing} is a crowd-sourced dataset. It consists of multi-turn dialogues that are based on given persona information. Table ? shows some data instances. We randomly sample 200 persona with corresponding dialogues for annotation. We conduct a selectively masked sensitive information and then dialogue datasets.

\textit{}

\subsubsection{Automatic Annotation} We adopt two automatic evaluation methods, one based on LLM and another one based on an observation that sensitive span are in lower probability distribution than common phrases. We 

\paragraph{LLM based annotation}
Shortcoming of LLM based annotation is that: 1) The annotation quality of LLM based method is uncontrollable. It is not easy to verify if all the sensitive information has been annotates, and is the generated sensitive span is faithful to the original context which needs post-processing after LLM annotation. 

\paragraph{Probability based annotation}

\subsubsection{Human Annotation}
The purposes of human annotation are summarized as the follows: 1) to have a high-quality of annotated datasets to assistant the assessment of unlearning or related methods. 2) to compare with automatically annotated results, thus to have a overall estimation of the quality of the automatic annoated datasets.

We 



\paragraph{}

\subsection{Proposed Unlearning Evaluation Metrics }

\section{Statistics of the Annotated Datasets}
\paragraph{Analysis of Annotated Datasets based on three methods}

\paragraph{Comparison between annotated sensitive information with Named-entity recognition}
\paragraph{}

\subsection{Quantitative Comparison with Previous Evaluation Metrics}






==> sections/evaluation_metrics.tex <==
\section{Evaluation Metrics}


==> tables/forgetting_threshold.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{1mm}\small
\begin{center}
% \resizebox{\linewidth}{!}{
\begin{tabular}{l|cc}
\toprule[1.0pt]
\textbf{Model(Size)}  &$\textbf{\textsc{EL}}_{10}$(\%) &\textbf{MA(\%)} \\
\midrule[0.5pt]
\textsc{GPT-Neo} (125M) & $4.99$ & $29.94$\\
    \textsc{GPT-Neo} (1.3B) & $5.68$ & $33.27$\\
    \textsc{GPT-Neo} (2.7B) & $5.53$ & $34.02$ \\
\bottomrule[1.0pt]
\end{tabular}
% }
\end{center}
\vskip -1em
\caption{\label{tab:forgetting_threshold} Empirical threshold calculated by 10,000 samples from Pile validation corpus \cite{jang2022knowledge}. 
}
\vskip -1em
\end{table}

==> tables/main_results_classification.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{1.1mm}\small
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \begin{center}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{ll|cccc|c|cc|ccccc|c}
                \toprule
                \multirow{2}{*}{Models} & & \multicolumn{4}{c}{\tabincell{c}{Forget Evaluation}} & \multicolumn{9}{c}{\tabincell{c}{Classification Test Set Evaluation}} \\
                \cmidrule(lr){3-6}\cmidrule(lr){7-14}\cmidrule(lr){15-15}
                & & EL & MA & S-EL & S-MA & Hella. & Wino. & COPA  & ARC-E & ARC-C & Piqa  & MathQ & PubQ & Avg. \\
                \midrule
                \rowcolor[rgb]{0.93,0.93,0.93}
                \multirow{4}{*}{\tabincell{l}{GPT-Neo \\ 125M}} & Original &31.5 &76.9 &22.0 &62.4  &28.2 &51.5 &60.2 &46.1 &20.3 &63.4 &22.5 &57.2  &43.7 \\
                & \textsc{Kul} &0.2 &26.8 & 1.3 &22.9  &27.1 &52.5 &50.8 &38.5 &19.1 &60.1 &22.1 &57.2  & 40.9\\
                & \shortname &1.0 &29.5 &0.3 &16.1  &27.5 &49.3 &55.5 &37.9 &25.0 &58.9 &20.8  &52.8 &41.0  \\
                \midrule
                \rowcolor[rgb]{0.93,0.93,0.93}
                \multirow{4}{*}{\tabincell{l}{GPT-Neo \\ 1.3B}} & Original &60.4 &91.1 &44.6 &81.6  &37.0 &54.5 &69.2 &56.6 &25.8 &70.3 &21.9 &53.4  &48.6 \\
                & \textsc{Kul} &0.3 &27.2 &1.4 &23.9  &36.7 &55.6 &69.2 &54.0 &25.4 &70.1 &21.6 &52.8  &48.2 \\
                % & $\Delta$(\textsc{Kul},Ori) &- &- &- &-  &($\downarrow0.6$) &($\uparrow0.3$) &($\downarrow0.6$) &($\downarrow2.9$) &($\uparrow0.4$) &($\downarrow1.0$) &(0.0) &($\downarrow1.0$)  &($\downarrow0.6$) \\
                & \shortname &0.6 &29.4 &1.9 &23.6  &36.6 &55.0 &69.3 &54.6 &25.8 &69.5 &21.8  &51.4 & 48.0\\
                \midrule
                \rowcolor[rgb]{0.93,0.93,0.93}
                \multirow{4}{*}{\tabincell{l}{GPT-Neo \\ 2.7B}} & Original &66.6 &93.1 &49.5 &82.5  &40.7 &55.9 &74.2 &59.6 &24.6 &72.9 &21.4 &56.6  &50.7 \\
                & \textsc{Kul} &0.5 &29.8 &1.7 &23.0  &40.8 &55.8 &67.3 &54.5 &29.8 &72.8 &21.5 & 56.9  &49.9 \\
                & \shortname &0.3 &18.6 &1.0 &14.6  &40.3 &55.4 & 70.5 &56.2 &27.2 &73.0 &22.0 & 56.7   &50.2 \\
                \bottomrule
            \end{tabular}
        }
    \end{center}
    % \vskip -1em
    \caption{\label{tab:main_results_classification} Full comparison results (in \%) on forget set ($d$=32) and 8 classification datasets. }
    % \vskip -1em
\end{table*}




==> tables/main_results_dialogue.tex <==

\begin{table*}[t]
\setlength{\tabcolsep}{1.1mm}\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{ll|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Models} & & \multicolumn{10}{c}{ \tabincell{c}{Dialogue Test Set Evaluation}}
\\
\cmidrule(lr){3-12}
&& \multicolumn{2}{c}{ \tabincell{c}{WoW}} & \multicolumn{2}{c}{ \tabincell{c}{ED}} & \multicolumn{2}{c}{ \tabincell{c}{BST}}  & \multicolumn{2}{c}{ \tabincell{c}{WoI}} &  \multicolumn{2}{c}{ \tabincell{c}{Avg.}}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
& &F1 & PPL &F1 & PPL &F1 & PPL &F1 & PPL &F1 & PPL \\
\midrule
\rowcolor[rgb]{0.93,0.93,0.93}
                \multirow{5}{*}{\tabincell{l}{GPT-Neo \\ 125M}} & Original  &10.5 &45.5 &8.4 &41.1 &9.6 &44.9 &11.2 &42.8  &7.4 &43.6 \\
\midrule
& \textsc{Kul}   &1.3 &654.4 &1.2 &438.1 &0.7 &526.1 &1.1 &537.8  &1.1 &539.1 \\
% & \;\;$\Delta$(\textsc{Kul},Ori)  &($\downarrow$5.9) & &($\downarrow$5.5) & &($\downarrow$7.5) & &($\downarrow$8.4) &  &($\downarrow$6.8) & \\
& \shortname  &8.1 &214.9 &7.0 &152.8 &7.2 &185.0 &8.7 &166.6  &7.8 &179.8 \\

% & \;\;$\Delta$(\shortname,Ori) & & & & & & & &  & & \\
\midrule
\rowcolor[rgb]{0.93,0.93,0.93}
                \multirow{5}{*}{\tabincell{l}{GPT-Neo \\ 1.3B}} &Original  &12.7 &26.5 &10.5 &25.3 &12.1 &27.0 &13.8 &25.0  &12.3 &26.0 \\
\midrule
& \textsc{Kul} &11.2 &33.0 &9.3 &31.9 &9.9 &33.6 &11.2 &31.1 &10.4 &32.4 \\
% & \;\;$\Delta$(\textsc{Kul},Ori) & & & & & & & &  & & \\
& \shortname  &12.3 &28.9 &10.2 &27.9 &10.7 &29.4 &12.3 &27.0  &11.4 &28.3 \\
% & \;\;$\Delta$(\shortname,Ori) & & & & & & & &  & & \\
\midrule
\rowcolor[rgb]{0.93,0.93,0.93}
                \multirow{5}{*}{\tabincell{l}{GPT-Neo \\ 2.7B}} &Original  &12.3 &23.5 &10.8 &22.9 &12.5 &24.0 &13.5 &22.6  &12.3 &23.3 \\
\midrule
& \textsc{Kul} &10.8 &30.8 &8.8 &29.7 &9.7 &30.9 &10.9 &29.0  &10.1 &30.1 \\
% & \;\;$\Delta$(\textsc{Kul},Ori) & & & & & & & &  & & \\
& \shortname  &11.3 &27.0 &9.2 &26.6 &11.0 &27.3 &12.0 &26.0  &10.9 &26.7 \\
% & \;\;$\Delta$(\shortname,Ori) & & & & & & & &  & & \\

\bottomrule
\end{tabular}
}
\end{center}
% \vskip -1em
\caption{\label{tab:main_results_dialogue} 
Full comparison results (in \%) with $d$=32 setting on 4 dialogue datasets.  
}
% \vskip -1em
\end{table*}

==> tables/unlearning_data_comparison.tex <==
\begin{table*}[t!]
\centering
\fontsize{7}{9}\selectfont
\caption{\footnotesize Forgetting Threshold for \textsc{GPT-Neo} LMs}
\begin{tabular*}{0.4\columnwidth}{l|cc}
    \toprule
    \multirowcell{2}{\textbf{Model (Size)}} & $\textbf{\textsc{EL}}_{10}$ (\%)  & \textbf{MA(\%)} \\
        & \textbf{Threshold} & \textbf{Threshold} \\
    \midrule
    \textsc{GPT-Neo} (125M) & $4.99$ & $29.94$\\
    \textsc{GPT-Neo} (1.3B) & $5.68$ & $33.27$\\
    \textsc{GPT-Neo} (2.7B) & $5.53$ & $34.02$ \\
    \bottomrule
\end{tabular*}
\label{table:threshold}
\end{table*}
